Mode changing, subpulse drifting and nulling in four component conal pulsar PSR J2321+6024

In this study, we report on a detailed single pulse polarimetric analysis of the radio emission from the pulsar J2321+6024 (B2319+60) observed with the Giant Metrewave Radio Telescope, over wide frequencies ranging between 300 to 500 MHz and widely separated observing sessions. The pulsar profile shows the presence of four distinct conal components and belongs to a small group of pulsars classified as a conal quadrupole profile type. The single pulse sequence reveals the presence of three distinct emission modes, A, B, and ABN showing subpulse drifting. Besides, there were sequences when the pulsar did not show any drifting behaviour suggesting the possibility of a new emission state, which we have termed as mode C. The evolution of the mode changing behavior was seen during the different observing sessions with different abundance as well as the average duration of the modes seen on each date. The drifting periodicities were 7.8$\pm$0.3 $P$, 4.3$\pm$0.4 $P$, and 3.1$\pm$0.2 $P$ in the modes A, B and ABN respectively, and showed large phase variations within the mode profile. The pulsar also showed the presence of orthogonal polarization modes, particularly in the leading and trailing components, which has different characteristics for the stronger and weaker pulses. However, no correlation was found between the emission modes and their polarization behavior, with the estimated emission heights remaining roughly constant throughout. We have used the Partially Screened Gap model to understand the connection between drifting, mode changing, and nulling.

==> table_Drift.tex <==
\begin{table}
\centering
\caption{Measuring Subpulse Drifting Periodicity in Mode A}
\label{tab:Drift-modeA}
\begin{tabular}{ccccc}
\hline
Pulse range  & $f_p$ & $FWHM$ & $S$ & P$_3$  \\
             & ($cy/P$) & ($cy/P$) &   &  (P) \\
\hline
            &   & \underline{06 Nov, 2017.} &   &  \\
            &   &                          &   &  \\
  14 - 117  & 0.124$\pm$0.006 & 0.013 & 55.9 & 8.05$\pm$0.37 \\
 404 - 464  & 0.125$\pm$0.012 & 0.029 & 22.7 & 8.00$\pm$0.79 \\
 503 - 578  & 0.131$\pm$0.017 & 0.039 & 16.4 & 7.63$\pm$0.97 \\
 659 - 791  & 0.129$\pm$0.004 & 0.009 & 82.2 & 7.76$\pm$0.24 \\
 904 - 966  & 0.128$\pm$0.010 & 0.024 & 29.0 & 7.82$\pm$0.61 \\
1176 - 1242 & 0.120$\pm$0.009 & 0.021 & 31.6 & 8.30$\pm$0.61 \\
1531 - 1583 & 0.125$\pm$0.010 & 0.024 & 26.5 & 7.99$\pm$0.65 \\
1854 - 1988 & 0.123$\pm$0.008 & 0.019 & 37.3 & 8.10$\pm$0.54 \\
2058 - 2104 & 0.128$\pm$0.014 & 0.034 & 18.6 & 7.84$\pm$0.89 \\
            &     &       &      &  \\
            &     & \underline{16 Nov, 2018.} &      &  \\
            &                 &       &      &  \\
 182 - 270  & 0.122$\pm$0.011 & 0.026 & 27.4 & 8.18$\pm$0.74 \\
 675 - 740  & 0.123$\pm$0.014 & 0.033 & 19.8 & 8.16$\pm$0.94 \\
 956 - 1025 & 0.129$\pm$0.008 & 0.019 & 33.9 & 7.74$\pm$0.49 \\
1444 - 1531 & 0.127$\pm$0.010 & 0.024 & 28.7 & 7.90$\pm$0.63 \\
2308 - 2373 & 0.146$\pm$0.011 & 0.026 & 25.7 & 6.87$\pm$0.52 \\
2500 - 2544 & 0.136$\pm$0.017 & 0.041 & 14.4 & 7.33$\pm$0.94 \\
            &     &       &      &  \\
            &     & \underline{22 July, 2019.} &      &  \\
            &     &       &      &  \\
 112 - 163  & 0.126$\pm$0.019 & 0.044 & 15.8 & 7.93$\pm$1.18 \\
 567 - 648  & 0.134$\pm$0.006 & 0.014 & 52.9 & 7.48$\pm$0.33 \\
 733 - 778  & 0.121$\pm$0.017 & 0.041 & 16.4 & 8.28$\pm$1.19 \\
 878 - 963  & 0.127$\pm$0.006 & 0.015 & 50.5 & 7.88$\pm$0.39 \\
1926 - 1975 & 0.131$\pm$0.013 & 0.031 & 23.0 & 7.64$\pm$0.76 \\
2089 - 2128 & 0.124$\pm$0.011 & 0.026 & 26.2 & 8.04$\pm$0.72 \\
            &     &       &      &  \\
\hline
\end{tabular}
\end{table}


==> table_Emission_height.tex <==

\begin{table*}
\centering
\caption{Profile Widths and Emission Heights for 22 July, 2019 observations (see section~\ref{Emission height and geometry} for details).}
\label{tab:Profheight}
\begin{tabular}{cccccccccccc}
\hline
  Mode & Band & W$_{5\sigma}$ & W$_{10}$ & W$_{50}$ & W$_{sep}^{out}$ &  W$_{sep}^{in}$  & $\phi_{\circ}$ & $\phi_{t}^{5\sigma}$ & $\phi_{l}^{5\sigma}$ & $\Delta \phi$ & h$_{A/R}$\\
   &       &           &           &           &           &                 &           &                &        \\ 
   & (MHz) & ($\degr$) & ($\degr$) & ($\degr$) & ($\degr$) & ($\degr$) & ($\degr$) & ($\degr$)  & ($\degr$) & ($\degr$) & (km)\\ 
\hline
  A  & 300--330 & 30.9$\pm$0.2 & 29.0$\pm$0.2 & 23.5$\pm$0.2 &   19.6$\pm$0.2 & 6.4$\pm$0.2 & -8.7$\pm$0.3 & 15.1$\pm$0.3 & -15.8$\pm$0.3 & 0.7$\pm$0.3 & 329$\pm$141  \\
     & 330--360 & 35.8$\pm$0.2 & 27.9$\pm$0.2 & 23.2$\pm$0.2 &   19.6$\pm$0.2 & 5.6$\pm$0.2 & -8.7$\pm$0.2 & 17.2$\pm$0.2 & -18.5$\pm$0.2 & 1.3$\pm$0.2 & 611$\pm$94 \\
     & 379--409 & 34.2$\pm$0.2 & 27.1$\pm$0.2 & 22.4$\pm$0.2 &   17.6$\pm$0.2 & 4.4$\pm$0.2 & -8.6$\pm$0.2 & 16.0$\pm$0.3 & -18.2$\pm$0.3 & 2.2$\pm$0.3 & 1034$\pm$141 \\
     & 418--448 & 29.0$\pm$0.2 & 26.5$\pm$0.2 & 22.0$\pm$0.2 &   17.6$\pm$0.2 & 4.3$\pm$0.2 & -7.5$\pm$0.2 & 13.4$\pm$0.3 & -15.6$\pm$0.3 & 2.2$\pm$0.3 & 1034$\pm$141 \\
     & 455--485 & 31.8$\pm$0.2 & 25.9$\pm$0.2 & 21.7$\pm$0.2 &   17.6$\pm$0.2 & 4.4$\pm$0.2 & -7.8$\pm$0.2 & 15.4$\pm$0.2 & -16.4$\pm$0.2 & 1.0$\pm$0.2 & 470$\pm$94 \\
     &          &              &              &              &              &             &              &               &              &            \\
  B  & 300--330 & 32.3$\pm$0.2 & 32.2$\pm$0.2 & 24.2$\pm$0.2 &   20.4$\pm$0.2 & ---   & -9.1$\pm$0.6  & 14.0$\pm$0.6 & -18.3$\pm$0.6 & 4.3$\pm$0.6 & 2021$\pm$282  \\
     & 330--360 & 33.6$\pm$0.2 & 28.9$\pm$0.2 & 23.7$\pm$0.2 &   19.8$\pm$0.2 & ---   & -8.6$\pm$0.2   & 15.9$\pm$0.2 & -17.7$\pm$0.2 & 1.8$\pm$0.2 & 846$\pm$94 \\
     & 379--409 & 32.2$\pm$0.2 & 27.8$\pm$0.2 & 22.9$\pm$0.2 &   18.7$\pm$0.2 & ---   & -8.4$\pm$0.2  & 15.0$\pm$0.2 & -17.1$\pm$0.2 & 2.1$\pm$0.2 & 987$\pm$94 \\
     & 418--448 & 30.0$\pm$0.2 & 27.5$\pm$0.2 & 22.4$\pm$0.2 &   18.7$\pm$0.2 & ---   & -8.5$\pm$0.3  & 13.5$\pm$0.3 & -16.5$\pm$0.3 & 3.0$\pm$0.3 & 1410$\pm$141 \\
     & 455--485 & 30.1$\pm$0.2 & 26.8$\pm$0.2 & 22.3$\pm$0.2 &   18.5$\pm$0.2 & ---   & -8.5$\pm$0.2 & 14.1$\pm$0.2 & -16.0$\pm$0.2 & 1.9$\pm$0.2 & 893$\pm$94 \\
     &          &              &              &              &              &       &              &                &             &            \\
          
 ABN & 300--330 & 26.7$\pm$0.2 &   ---        & 24.0$\pm$0.2 & 20.1$\pm$0.2 &   ---  & 8.8$\pm$2.8  & 13.1$\pm$0.2 & -13.6$\pm$0.2 &  ---         & ---     \\
     & 330--360 & 32.3$\pm$0.2 & 29.5$\pm$0.2 & 23.7$\pm$0.2 & 19.9$\pm$0.2 &   ---  & 9.1$\pm$2.7  & 16.2$\pm$0.2 & -16.1$\pm$0.2 &  ---         & ---     \\
     & 379--409 & 30.1$\pm$0.2 & 27.8$\pm$0.2 & 22.9$\pm$0.2 & 18.5$\pm$0.2 &   ---  & 9.3$\pm$2.0  & 14.3$\pm$0.2 & -15.8$\pm$0.2 &  ---         & ---     \\
     & 418--448 & 28.4$\pm$0.2 &  ---         & 22.4$\pm$0.2 & 18.5$\pm$0.2 &   ---  & 10.0$\pm$2.0 & 13.1$\pm$0.2 & -15.3$\pm$0.2 &  ---         & ---     \\
     & 455--485 & 28.2$\pm$0.2 & 26.7$\pm$0.2 & 22.0$\pm$0.2 & 18.0$\pm$0.2 &   ---  & 9.5$\pm$2.0  & 13.0$\pm$0.2 & -15.3$\pm$0.2 &  ---         & ---      \\
     &          &              &              &              &              &        &              &               &              &          \\
  C  & 300--330 & 31.7$\pm$0.2 & 30.3$\pm$0.2 & 24.9$\pm$0.2 & 20.2$\pm$0.2 &   ---    & -9.9$\pm$0.2 & 15.3$\pm$0.2 & -16.4$\pm$0.2 & 1.1$\pm$0.2 & 517$\pm$94  \\
     & 330--360 & 34.4$\pm$0.2 & 29.3$\pm$0.2 & 24.3$\pm$0.2 & 19.8$\pm$0.2 &   ---    & -9.7$\pm$0.2 & 16.8$\pm$0.2 & -17.5$\pm$0.2 & 0.7$\pm$0.2 & 329$\pm$94 \\
     & 379--409 & 33.6$\pm$0.2 & 28.6$\pm$0.2 & 23.7$\pm$0.2 & 18.8$\pm$0.2 &   ---    & -8.9$\pm$0.2 & 16.4$\pm$0.2 & -17.2$\pm$0.2 & 0.8$\pm$0.2 & 376$\pm$94 \\
     & 418--448 & 30.1$\pm$0.2 & 28.1$\pm$0.2 & 23.2$\pm$0.2 & 18.5$\pm$0.2 &   ---    & -9.1$\pm$0.3 & 15.0$\pm$0.3 & -15.1$\pm$0.3 & --- & --- \\
     & 455--485 & 31.8$\pm$0.2 & 27.5$\pm$0.2 & 22.9$\pm$0.2 & 18.2$\pm$0.2 &   ---    & -8.9$\pm$0.2 & 16.0$\pm$0.3 & -15.8$\pm$0.3 &  --- & --- \\
     &          &              &              &              &              &             &              &                &              &         \\
 All & 300--330 & 33.4$\pm$0.2 & 29.5$\pm$0.2 & 24.0$\pm$0.2 & 19.8$\pm$0.2 &  ---  & -9.0$\pm$0.2  &  15.8$\pm$0.2 & -17.6$\pm$0.2 & 1.8$\pm$0.2 & 846$\pm$94  \\
     & 330--360 & 36.2$\pm$0.2 & 28.6$\pm$0.2 & 23.5$\pm$0.2 & 19.0$\pm$0.2 &  ---  & -8.7$\pm$0.2  & 17.6$\pm$0.2 & -18.6$\pm$0.2 & 1.0$\pm$0.2 & 470$\pm$94 \\
     & 379--409 & 35.3$\pm$0.2 & 27.6$\pm$0.2 & 22.8$\pm$0.2 & 18.5$\pm$0.2 &  ---  & -8.6$\pm$0.2  & 16.9$\pm$0.2 & -18.4$\pm$0.2 & 1.5$\pm$0.2 & 705$\pm$94 \\
     & 418--448 & 31.5$\pm$0.2 & 26.8$\pm$0.2 & 22.4$\pm$0.2 & 18.4$\pm$0.2 &  ---  & -8.6$\pm$0.2  & 14.8$\pm$0.2 & -16.8$\pm$0.2 & 2.0$\pm$0.2 & 940$\pm$94 \\
     & 455--485 & 33.3$\pm$0.2 & 26.5$\pm$0.2 & 22.0$\pm$0.2 & 17.7$\pm$0.2 &  ---  & -7.9$\pm$0.2  & 16.1$\pm$0.2 & -17.2$\pm$0.2 & 1.1$\pm$0.2 & 517$\pm$94 \\
     &          &              &              &              &              &             &              &                &              &          \\
     
\hline    
\end{tabular}
\end{table*}

==> table_Mode.tex <==
\begin{table*}
\centering
\caption{List of the pulse range and duration (Len) of the four emission modes, A, B, ABN and C during each observing session.}
\label{tab:modelist}
\begin{tabular}{c@{\hskip5pt}c@{\hskip5pt}c@{\hskip18pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip18pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c}
\hline
\multicolumn{3}{c}{4 Nov, 2017} & \multicolumn{6}{c}{16 Nov, 2018} & \multicolumn{6}{c}{22 July, 2019} \\
\hline
Pulse & Mode & Len & Pulse & Mode & Len & Pulse & Mode & Len & Pulse & Mode & Len & Pulse & Mode & Len \\
(P) &  & (P) & (P) &  & (P) & (P) &  & (P) & (P) &  & (P) & (P) &  & (P) \\
\hline
   14 - 116  &  A  & 103 &    1 - 10   &  B  & 10 & 1418 - 1425 &  B  & ~8 &    1 - 35   & ABN & 35 & 1477 - 1481 & ABN & ~5 \\
  120 - 127  &  B  & ~~8 &   17 - 26   &  B  & 10 & 1426 - 1438 & ABN & 13 &   51 - 68   & ABN & 18 & 1496 - 1508 &  B  & 13 \\
  129 - 134  &  C  & ~~6 &   27 - 34   &  C  & ~8 & 1443 - 1530 &  A  & 88 &   84 - 99   & ABN & 16 & 1519 - 1530 &  B  & 12 \\
  155 - 184  &  C  & ~30 &   65 - 72   &  C  & ~8 & 1538 - 1552 &  B  & 15 &  111 - 162  &  A  & 52 & 1537 - 1543 &  B  & ~7 \\
  187 - 207  & ABN & ~21 &   77 - 103  &  A  & 27 & 1555 - 1560 &  C  & ~6 &  177 - 195  &  A  & 19 & 1544 - 1548 & ABN & ~5 \\
  231 - 259  &  A  & ~29 &  152 - 169  &  C  & 18 & 1561 - 1574 & ABN & 14 &  197 - 208  &  B  & 12 & 1558 - 1586 &  A  & 29 \\
  264 - 315  &  C  & ~52 &  181 - 269  &  A  & 89 & 1589 - 1634 &  C  & 46 &  221 - 230  & ABN & 10 & 1596 - 1606 &  A  & 11 \\
  332 - 344  &  A  & ~13 &  272 - 303  &  B  & 32 & 1656 - 1666 &  C  & 11 &  240 - 250  &  A  & 11 & 1708 - 1721 &  B  & 14 \\
  370 - 385  & ABN & ~16 &  309 - 317  &  B  & ~9 & 1674 - 1683 &  B  & 10 &  251 - 257  & ABN & ~7 & 1731 - 1754 &  A  & 24 \\
  388 - 398  &  C  & ~11 &  318 - 328  & ABN & 11 & 1692 - 1720 &  A  & 29 &  265 - 273  &  A  & ~9 & 1757 - 1787 &  B  & 31 \\
  403 - 463  &  A  & ~61 &  349 - 389  &  A  & 41 & 1722 - 1734 &  B  & 13 &  284 - 303  &  A  & 20 & 1790 - 1794 & ABN & ~5 \\
  469 - 477  &  B  & ~~9 &  401 - 429  &  C  & 29 & 1758 - 1776 &  B  & 19 &  327 - 363  &  A  & 37 & 1811 - 1815 & ABN & ~5 \\
  496 - 577  &  A  & ~83 &  447 - 478  &  A  & 32 & 1790 - 1799 &  B  & 10 &  374 - 383  &  A  & 10 & 1838 - 1848 &  B  & 11 \\
  585 - 601  &  C  & ~17 &  487 - 497  &  A  & 11 & 1803 - 1808 & ABN & ~6 &  384 - 391  & ABN & ~8 & 1849 - 1860 &  A  & 12 \\
  604 - 624  & ABN & ~21 &  503 - 511  & ABN & ~9 & 1837 - 1849 &  A  & 13 &  439 - 447  &  A  & ~9 & 1902 - 1981 &  A  & 80 \\
  658 - 804  &  A  & 146 &  546 - 559  &  B  & 14 & 1856 - 1865 &  C  & 10 &  455 - 466  &  A  & 12 & 1989 - 2018 &  B  & 30 \\
  810 - 820  &  B  & ~11 &  562 - 573  & ABN & 12 & 1880 - 1890 &  B  & 11 &  477 - 500  &  B  & 24 & 2026 - 2034 &  B  & ~9 \\
  839 - 850  &  B  & ~12 &  631 - 644  &  B  & 14 & 2013 - 2095 &  C  & 83 &  501 - 517  &  C  & 17 & 2062 - 2085 &  B  & 24 \\
  854 - 862  & ABN & ~~9 &  645 - 657  & ABN & 13 & 2096 - 2110 &  B  & 15 &  528 - 537  &  C  & 10 & 2088 - 2127 &  A  & 40 \\
  896 - 979  &  A  & ~84 &  674 - 740  &  A  & 67 & 2115 - 2129 & ABN & 15 &  566 - 649  &  A  & 84 & 2134 - 2140 &  B  & ~7 \\
  980 - 1003 &  C  & ~24 &  747 - 757  &  B  & 11 & 2150 - 2180 &  C  & 31 &  662 - 674  &  B  & 13 & 2162 - 2191 &  A  & 30 \\
 1042 - 1081 &  C  & ~40 &  761 - 768  & ABN & ~8 & 2201 - 2221 &  A  & 21 &  678 - 686  & ABN & ~9 & 2192 - 2208 &  B  & 17 \\
 1117 - 1138 &  C  & ~22 &  776 - 788  &  A  & 13 & 2229 - 2241 &  B  & 13 &  704 - 714  &  C  & 11 & 2231 - 2267 &  A  & 37 \\
 1175 - 1241 &  A  & ~67 &  791 - 809  &  B  & 19 & 2242 - 2250 & ABN & ~9 &  732 - 777  &  A  & 46 & 2284 - 2299 & ABN & 16 \\
 1248 - 1264 &  B  & ~17 &  813 - 820  & ABN & ~8 & 2257 - 2265 &  C  & ~9 &  778 - 791  &  B  & 14 & 2318 - 2327 &  B  & 10 \\
 1267 - 1337 &  C  & ~71 &  860 - 883  &  A  & 24 & 2286 - 2372 &  A  & 87 &  800 - 817  &  C  & 18 & 2330 - 2339 & ABN & 10 \\
 1358 - 1389 &  C  & ~32 &  892 - 904  &  A  & 13 & 2375 - 2390 &  B  & 16 &  828 - 845  &  A  & 18 & 2348 - 2357 & ABN & 10 \\
 1431 - 1443 &  A  & ~13 &  912 - 926  &  B  & 15 & 2406 - 2412 &  C  & ~7 &  852 - 869  &  B  & 18 &             &     &    \\
 1468 - 1475 &  C  & ~~8 &  927 - 938  & ABN & 12 & 2413 - 2425 & ABN & 13 &  877 - 962  &  A  & 86 &             &     &    \\
 1481 - 1499 &  B  & ~19 &  945 - 1032 &  A  & 88 & 2430 - 2440 &  A  & 11 &  973 - 1053 &  C  & 81 &             &     &    \\
 1521 - 1646 &  A  & 126 & 1033 - 1044 &  B  & 12 & 2448 - 2454 &  C  & ~7 & 1062 - 1070 & ABN & ~9 &             &     &    \\
 1647 - 1660 &  B  & ~14 & 1073 - 1086 &  B  & 14 & 2474 - 2543 &  A  & 70 & 1086 - 1102 &  A  & 17 &             &     &    \\
 1662 - 1682 &  C  & ~21 & 1087 - 1099 & ABN & 13 & 2557 - 2597 &  A  & 41 & 1120 - 1132 &  B  & 13 &             &     &    \\
 1696 - 1706 &  B  & ~11 & 1130 - 1138 &  A  & ~9 &             &     &    & 1133 - 1139 & ABN & ~7 &             &     &    \\
 1707 - 1721 & ABN & ~15 & 1149 - 1161 &  A  & 13 &             &     &    & 1150 - 1160 &  B  & 11 &             &     &    \\
 1739 - 1750 &  B  & ~12 & 1177 - 1186 &  C  & 10 &             &     &    & 1167 - 1184 & ABN & 18 &             &     &    \\
 1761 - 1787 &  C  & ~27 & 1195 - 1212 &  B  & 18 &             &     &    & 1185 - 1219 &  A  & 35 &             &     &    \\
 1800 - 1812 &  B  & ~13 & 1221 - 1254 &  B  & 34 &             &     &    & 1221 - 1245 &  B  & 25 &             &     &    \\
 1813 - 1819 & ABN & ~~7 & 1255 - 1260 & ABN & ~6 &             &     &    & 1251 - 1277 &  C  & 27 &             &     &    \\
 1826 - 1835 &  C  & ~10 & 1281 - 1297 &  B  & 17 &             &     &    & 1297 - 1386 &  C  & 90 &             &     &    \\
 1847 - 2000 &  A  & 154 & 1305 - 1341 &  A  & 37 &             &     &    & 1395 - 1405 &  C  & 11 &             &     &    \\
 2004 - 2012 &  C  & ~~9 & 1351 - 1358 &  B  & ~8 &             &     &    & 1406 - 1415 & ABN & 10 &             &     &    \\
 2023 - 2035 & ABN & ~13 & 1364 - 1370 & ABN & ~7 &             &     &    & 1433 - 1437 &  C  & ~5 &             &     &    \\
 2043 - 2054 &  C  & ~12 & 1379 - 1387 & ABN & ~9 &             &     &    & 1444 - 1461 &  A  & 18 &             &     &    \\ 
 2058 - 2112 &  A  & ~55 & 1398 - 1410 &  A  & 13 &             &     &    & 1466 - 1476 &  B  & 11 &             &     &    \\
             &     &     &             &     &    &             &     &    &             &     &    &             &     &    \\
\hline
\end{tabular}
\end{table*}

